JUNO Conceptual Design Report

The Jiangmen Underground Neutrino Observatory (JUNO) is proposed to determine the neutrino mass hierarchy using an underground liquid scintillator detector. It is located 53 km away from both Yangjiang and Taishan Nuclear Power Plants in Guangdong, China. The experimental hall, spanning more than 50 meters, is under a granite mountain of over 700 m overburden. Within six years of running, the detection of reactor antineutrinos can resolve the neutrino mass hierarchy at a confidence level of 3-4$\sigma$, and determine neutrino oscillation parameters $\sin^2\theta_{12}$, $\Delta m^2_{21}$, and $|\Delta m^2_{ee}|$ to an accuracy of better than 1%. The JUNO detector can be also used to study terrestrial and extra-terrestrial neutrinos and new physics beyond the Standard Model. The central detector contains 20,000 tons liquid scintillator with an acrylic sphere of 35 m in diameter. $\sim$17,000 508-mm diameter PMTs with high quantum efficiency provide $\sim$75% optical coverage. The current choice of the liquid scintillator is: linear alkyl benzene (LAB) as the solvent, plus PPO as the scintillation fluor and a wavelength-shifter (Bis-MSB). The number of detected photoelectrons per MeV is larger than 1,100 and the energy resolution is expected to be 3% at 1 MeV. The calibration system is designed to deploy multiple sources to cover the entire energy range of reactor antineutrinos, and to achieve a full-volume position coverage inside the detector. The veto system is used for muon detection, muon induced background study and reduction. It consists of a Water Cherenkov detector and a Top Tracker system. The readout system, the detector control system and the offline system insure efficient and stable data acquisition and processing.

==> AssemblyAndInstallation/chapter12.tex <==
\chapter{AssemblyAndInstallation}
\label{ch:AssemblyAndInstallation}


\input{AssemblyAndInstallation/chapter12.1.tex}

\input{AssemblyAndInstallation/chapter12.2.tex}

\input{AssemblyAndInstallation/chapter12.3.tex}

\input{AssemblyAndInstallation/chapter12.4.tex}

\input{AssemblyAndInstallation/chapter12.5.tex}



==> OfflineSoftwareAndComputing/data_proc_req.tex <==
\subsection{Data Process Requirement}

Data taking period of JUNO will start from 2019 and raw data it generates each year would be about 2PB. Raw data would be transferred to computing center of IHEP via dedicate network connection. A large scale offline computing platform is necessary for the computation of simulation and reconstruction. Besides, it will support analysis computation. The platform will also provide enough storage space for the raw data, Monte Carlo data and data archive. With the rough estimation, the scale of the platform would be 10,000 cpus/cores, 10PB disk storage and 30PB archive. 40Gbps bone switching network is the connection among computing nodes and storage servers. To promote the data process speed, the platform would integrate computing resources of collaboration group members via distributed computation. Data would be shared and computation tasks would be dispatched to the sites included in the platform cooperatively. So JUNO puts forward high demands to data analysis process, data storage, data transfer and data share as the following four aspects.

\subsection{Data transferring requirement}
Data transfer and exchange system with features of high performance, high security and high availability is necessary. To guarantee the experiment data transferring from experiment site to IHEP data center in time, the system should monitor and trace the online status of data transferring and exchange and it should provide data transfer visualization interface. This could also guarantee the data dispatch and share in the collaborative group member sites smoothly.

\subsection{Computing Environment}

To guarantee JUNO data process smoothly, a 10,000 cpus/cores local cluster would be established. The collaboration group member would also provide computing resources according to the different cases. The platform includes not only local cluster, but remote resources from collaboration group member, who is responsible for the JUNO computation task either.

\subsection{Data Storage}

JUNO will generate huge experiment data. Data from experiment site should be transferred and stored at computing center of IHEP. The capacity of storage in IHEP would be 10 PB. It could support 10,000 cpus/cores concurrence access. Data migration between tape library and disk is transparent to users.

\subsection{Maintenance Monitoring and Service Support}
To guarantee the platform stable, an intelligent monitoring system would be developed and an information system aimed at infrastructure management should be established. The status of both platform and network connection should be monitored in a very fine grain control. The monitor tool could give the status assessment of the whole platform and give a tendency prediction and pre-warning for the relative services of the platform. A set of information management tools should be developed including conference support, document management and online-shift management etc.



==> PMT/AssemblyAndInstallation/chapter12.1.tex <==
\section{Introduction}

After the completion of civil construction, through systems integration, assembly, installation and commissioning, all subsystems will be formed as a whole JUNO detector.

In this process, we need to establish various engineering 
regulations and standards, and to coordinate subsystems' assembly, installation, testing and commissioning, especially their onsite work.

\subsection{Main Tasks}

Main tasks of the integration work include:
\begin{itemize}
\item To prepare plans and progress reports of each phase; 
\item To establish a project technology review system; 
\item To standardize the executive technology management system; 
\item To have strictly executive on-site work management system; 
\item To develop and specify security management system on-site; 
\item To prepare common tools and equipment for each system, and to guarantees project progress; 
\item To coordinate the installation progress of each system according to the on-site situation.
\end{itemize}

\subsection{Contents}

The work contents mainly include:
\begin{itemize}
\item To summarize the design, and review progress of each subsystem;
\item To organize preparation work for installation in the experiment region; 
\item To inspect and certify Surface Buildings, underground Tunnels, and Experiment Hall with relevant utilities;
\item To coordinate technology interfaces between key parts;
\item To coordinate the procedure of assembly and installation both on surface and underground;
\end{itemize}


==> PMT/AssemblyAndInstallation/chapter12.2.tex <==
\section{ Design Standards, Guidelines and Reviews}

\subsection{Introduction}

There will be a document to outline the mechanical design standards or guidelines that will be applied to the design work. It also describes the review process of engineering design that will be implemented to ensure that experimental equipment meets all requirements for performance and safety. The following is a brief summary of the guidance that all mechanical engineers/designers should follow in the process. For reasons ranging from local safety requirements to common sense practices, the following information should be understood and implemented in the design process.

\subsection{Institutional Standards}

When specific institutional design standards or guidelines exist, they should be followed. The guidelines outlined are not meant to replace but instead to supplement institutional guidelines. The majority of equipment and components built for the JUNO Experiment will be engineered and designed at home institutions, procured or fabricated at commercial vendors, then eventually delivered, assembled, installed, tested and operated at the JUNO Experimental facilities, Jiangmen, China. The funding agencies in other countries as well as Jiangmen, China will have some guidelines in this area, as would your home institutions. Where more than one set of guidelines exist, use whichever are the more stringent or conservative approaches.

\subsection{Design Loads}

The scope of engineering analysis should take handling, transportation, assembly and operational loads into account as well as thermal expansion considerations caused by potential temperature fluctuations.

For basic stability and a sensible practice in the design of experimental components an appropriate amount of horizontal load (0.10~g) should be applied.

In addition, seismic requirements for experimental equipment is based on a National Standard of People's Republic of China Code of Seismic Design of Buildings GB 50011-2010. At the location of the JUNO Experiment the seismic fortification intensity is grade 7 with a basic seismic acceleration of 0.10~g horizontal applied in evaluating structural design loads. A seismic hazard analysis should be performed and documented based on this local code. The minimum total design lateral seismic base shear force should be determined and applied to the component. The direction of application of seismic forces would be applied at the CG of the component that will produce the most critical load effect, or separately and independently in each of the two orthogonal directions. A qualitative seismic performance goal defines component functionality as: the component will remain anchored, but no assurance it will remain functional or easily repairable. Therefore, a seismic design factor of safety F.S. > 1 based on the Ultimate Strength of component materials would satisfy this goal.

Where an anticipated load path as designed above, allows the material to be subjected to stresses beyond the yield point of the material, redundancy in the support mechanism must be addressed in order to prevent a collapse mechanism of the structure from being formed.

The potential for buckling should also be evaluated. It should be
noted that a rigorous analytical seismic analysis may be performed
in lieu of the empirical design criteria. This work should be
properly documented for review by the Chief Engineer and appropriate
Safety Committee personnel.

\subsection{Materials Data}

All materials selected for component design must have their engineering data sources referenced along with those material properties used in any structural or engineering analysis; this includes fastener certification. There are many sources of data on materials and their properties that aid in the selection of an appropriate component material. There are many national and international societies and associations that compile and publish materials test data and standards. Problems frequently encountered in the purchasing, researching and selection of materials are the cross-referencing of designations and specification and matching equivalent materials from differing countries.

It is recommended that the American association or society standards be used in the
materials selection and specification process, or equivalency to these
standards must be referenced. Excellent engineering materials data have been
provided by the American Society of Metals or Machine Design Handbook Vol. 1-5 and
Mechanical Industry Publishing Co. in PRC, Vol 1-6, 2002, which are worth investigating.

\subsection{Analysis Methods}

The applicable factors of safety depend on the type of load(s) and how well they can be estimated, how boundary conditions have been approximated, as well as how accurate your method of analysis allows you to be.

\paragraph{Bounding Analyses:}
Bounding analysis or rough scoping analyses have proven to be
valuable tools. Even when computer modeling is in your plans, a
bounding analysis is a nice check to avoid gross mistakes. Sometimes
bounding analyses are sufficient. An example of this would be for
the case of an assembly fixture where stiffness is the critical
requirement. In this case where deflection is the over-riding
concern and the component is over-designed in terms of stress by a
factor of 10 or more, then a crude estimation of stress will
suffice.

\paragraph{Closed-Form Analytical Solutions:}
Many times when boundary conditions and applied loads are simple to
approximate, a closed-form or handbook solution can be found or developed. For
the majority of tooling and fixture and some non-critical experimental
components, these types of analyses are sufficient. Often, one of these
formulas can be used to give you a conservative solution very quickly, or a
pair of formulas can be found which represent upper and lower bounds of the
true deflections and stresses. Formulas for Stress and Strain by Roark and
Young is a good reference handbook for these solutions.

\paragraph{Finite Element Analysis:}
When the boundary conditions and loads get complex, or the correctness of the solution is critical, computer modeling is often required. If this is the case, there are several rules to follow, especially if you are not intimately familiar with the particular code or application.
\begin{enumerate}
\item Always bound the problem with an analytical solution or some other approximate means.
\item If the component is critical, check the accuracy of the code and application by modeling a similar problem for which you have an analytical or handbook solution.
\item Find a qualified person to review your results.
\item Document your assumptions and results.
\end{enumerate}

\subsection{Failure Criteria}

The failure criterion depends upon the application. Many factors such as the rate or frequency of load application, the material toughness (degree of ductility), the human or monetary risk of component failure as well as many other complications must be considered.

Brittle materials (under static loads, less than 5\% yield prior to failure), includes ceramics, glass, some plastics and composites at room temperature, some cast metals, and many materials at cryogenic temperatures. The failure criterion chosen depends on many factors so use your engineering judgment. In general, the Coulomb-Mohr or Modified Mohr Theory should be employed.

Ductile materials (under static loads, greater than 5\% yield prior to failure), includes most metals and plastics, especially at or above room temperature. The failure criterion chosen again ultimately rests with the cognizant engineer because of all the adverse factors that may be present. In general, the Distortion- Energy Theory, or von Mises-Hencky Theory (von Mises stresses), is most effective in predicting the onset of yield in materials. Slightly easier to use and a more conservative approach is the Maximum-Shear-Stress Theory.

\subsection{Factor of Safety}

Some institutions may have published guidelines which specifically discuss factors of safety for various applications. For the case where specific guidelines do not exist, the following may be used.

Simplistically, if F is the applied load (or S the applied stress),
and $F_f$ is the load at which failure occurs (or $S_s$ the stress
at which failure occurs), we can then define the factor of safety
(F.S.) as:
\begin{displaymath}
F.S. = F_{f} / F \quad\mathrm{or}\quad S_{s} / S
\end{displaymath}
The word failure, as it applies to engineering elements or systems, can be defined in a number of ways and depends on many factors. Discussion of failure criteria is presented in the previous section, but for the most common cases it will be the load at which yielding begins.

\subsection{Specific Safety Guidelines for JUNO}

Lifting and handling fixtures, shipping equipment, test stands, and fabrication
tooling where weight, size and material thickness do not affect the physical
capabilities of the detector, the appropriate F.S. should be at least 3. When
life safety is a potential concern, then a F.S. of 5 may be more appropriate.
Note that since the vast majority of this type of equipment is designed using
ductile materials, these F.S.'s apply to the material yield point. Experimental hardware that does not present a life safety or significant cost/schedule risk if failure occurs, especially where there is the potential for an increase in physics capabilities, the F.S. may be as low as 1.5. Many factors must be taken into account if a safety factor in this low level is to be employed: a complete analysis of worst case loads must be performed; highly realistic or else conservative boundary conditions must be applied; the method of analysis must yield accurate results; reliable materials data must be used or representative samples must be tested. If F.S.'s this low are utilized, the analysis and assumptions must be highly scrutinized. Guidelines for F.S. for various types of equipment are:

\begin{center}
\begin{tabular}{|p{3.5cm}|c|p{3.5cm}|}
\hline
Type of Equipment & Minimum F.S. & Notes \\
\hline
Lifting and handling & 3 - 5  & Where there is a risk to life
safety or to costly hardware,
choose F.S closer to 5. \\
\hline
Test stands, shipping and assembly fixtures. & 3 & \\
\hline
Experimental hardware & 1.5 - 3  & 1.5 is allowable for physics
capability and analysis where
method is highly refined \\
\hline
\end{tabular}
\end{center}

\subsection{Documentation}

It is not only good engineering practice to document the analysis, but it is an
ESH\&Q requirement for experimental projects. For this reason all major
components of JUNO Experiment will have their engineering analyses documented as Project Controlled Documents. Utilize your institutional documentation formats or use the following guidelines.
Calculations and analyses must
\begin{itemize}
\item Be hard copy documented.
\item Follow an easily understood logic and methodology.
\item Be legible and reproducible by photocopy methods.
\item Contain the following labeling elements.
    \begin{itemize}
    \item Title or subject
    \item Originators signature and date
    \item Reviewers signature and date
    \item Subsystem WBS number.
    \item Introduction, background and purpose.
    \item Applicable requirements, standards and guidelines.
    \item Assumptions (boundary conditions, loads, materials properties, etc.).
    \item Analysis method (bounding, closed form or FEA).
    \item Results (including factors of safety, load path and location of critical areas).
    \item Conclusions (level of conservatism, limitations, cautions or concerns).
    \item References (tech notes, textbooks, handbooks, software code, etc.).
    \item Computer program and version (for computer calculations)
    \item Filename (for computer calculations).
    \end{itemize}
\end{itemize}
\subsection{Design Reviews}

All experimental components and equipment whether engineered or
procured as turn-key systems will require an engineering design
review before procurement, fabrication, assembly or installation can
proceed. The L2 subsystem manager will request the design review
from the project management office, which will appoint a chair for
the review and develop a committee charge. The selected chair should
be knowledgeable in the engineering and technology, and where
practical, should not be directly involved in the engineering design
effort. With advice from the L2, the technical board and project
office chair appoints members to the review committee that have
experience and knowledge in the engineering and technology of the
design requiring review. At least one reviewer must represent ESH\&Q
concerns. The committee should represent such disciplines as:
\begin{itemize}
\item Science requirements
\item Design
\item Manufacturing
\item Purchasing
\item Operational user
\item Maintenance
\item Stress analysis
\item Assembly/installation/test
\item Electrical safety
\item ESH\&Q
\end{itemize}

For the JUNO project there will be a minimum of two engineering design reviews: Preliminary and Final. The preliminary usually takes place towards the end of the conceptual design phase when the subsystem has exhausted alternative designs and has made a selection based on value engineering. The L2 along with the chair ensures that the preliminary design review package contains sufficient information for the review along with:
\begin{itemize}
\item Agenda
\item Requirements documents
\item Review committee members and charge
\item Conceptual layouts
\item Science performance expectations
\item Design specifications
\item Supportive R\&D or test results
\item Summaries of calculations
\item Handouts of slides
\end{itemize}
A final design review will take place before engineering drawings or specifications are released for procurement or fabrication. The L2 along with the chair ensures that the final design review package contains sufficient information for the final review along with:
\begin{itemize}
\item Changes or revisions to preliminary design
\item Completed action items
\item Final assembly and detailed drawings
\item Final design specifications
\item Design calculations and analyses
\end{itemize}
The committee chair will ensure that meeting results are taken and recorded along with further action items. The committee and chair shall prepare a design review report for submittal to the project office in a timely manner which should include:
\begin{itemize}
\item Title of the review
\item Description of system or equipment
\item Copy of agenda
\item Committee members and charge
\item Presentation materials
\item Major comments or concerns of the reviewers
\item Action items
\item Recommendations
\end{itemize}
The project office will file the design review report and distribute copies to all reviewers and affected groups.


==> PMT/AssemblyAndInstallation/chapter12.3.tex <==
\section{On-site management}

According to the experience from the Daya Bay Experiment, an effective technology review system has been well practiced. In JUNO, we will take it as a good reference and carry out for standardized review from the start of all system design, scheme
argument, technology checks, we should also establish management system, to cover engineering drawing control, engineering change control procedure, and mechanical design standards, guidelines and reviews, etc.

To control on-site work process, proper process should be introduced as well as a management structure. Safety training and safety management structure should be also introduced. 




==> PMT/AssemblyAndInstallation/chapter12.4.tex <==
\section{Equipment and Tools Preparation on Site}

All of key equipment, devices and tools should be in place and get acceptance
for installation on site, including
\begin{itemize}
\item Cranes:
\begin{itemize}
\item 2 sets of bridge crane with 12T/5T load capacity, and lifting range should
cover any point for components delivery and installation in EH;
\item Several lifting equipment are needed in Surface Assembly areas, Assembly
Chamber underground, Storage area for Liquid Scintillation, and other Chambers
accordingly;
\end{itemize}
\item Removable lifting equipment: Forklifts, manual hydraulic carriages, carts,
etc.
\item Mobile vehicle for smaller items: Pickup van, battery car, and so on;
\item Several work aloft platform: Scissor lifts, Boom lifts, Scaffoldings and
Floating platforms, etc.
\item Common Tooling: complete kits of tool, fixtures, jigs, models, work-bench,
cabinets, and tables, etc.
\item Machine shop, Power equipment rooms, Control rooms are ready to be put into
use.
\item Safety measures and relevant equipment in place.
\end{itemize}


==> PMT/AssemblyAndInstallation/chapter12.5.tex <==
\section{Main Process of Installation}

Since there still are several optional design versions which could
be decided later, and different design could have different
requirements for installation, therefore, the specific installation
procedures will be established and developed later, here a very
rough installation procedure is given.
\begin{itemize}
\item Mounting, debugging, testing of basic utilities, such as, cranes, vertical
elevator, scaffoldings, test devices, etc.

\item Survey, alignment, and adjustment for tolerances of form and position, include,
embedded inserts, anchor plates, positioning holes, etc.

\item Mounting Bottom Structure of Veto Cherenkov detector on the floor of Water Pool.

\item Mounting anchor-plate for support poles of CD on the floor of Water Pool

\item Pre-mounting of Top Structure of Veto system along wall of Water Pool

\item Mount Substrate and Rails for Bridge over the water Pool edges

\item Mount Tyvek with support structure for Water Cherenkov Detector, and with PMT
positioning in the Water Pool

\item Installation for CD with its PMT system and cabling in Water Pool details will be established until design final selection.

\item Mount Calibration System

\item Mount Geomagnetic Shielding system around Central Detector in the Pool

\item Final installation for Tyvek and PMT of Veto system in the Pool

\item Mount a temporary protective cover on top of Pool, to prevent from anything
falling into Pool

\item Mount Bridge on the rails, and drive it closed

\item Mount Top Track Detector on Bridge and establish Electronic Room there

\item Have Cabling completion, and test to get normal signals
\item Check Grounding Electrode

\item Dry Run

\item Final Cleaning for Water Pool, then, drain out

\item Filling Water, LS, LAB (or Oil) evenly into Water Pool and CD

\item Mount Final Pool Cover, closed, and get fixation
\end{itemize}


==> PMT/AssemblyAndInstallation/chapter12.tex <==
\chapter{AssemblyAndInstallation}
\label{ch:AssemblyAndInstallation}


\input{AssemblyAndInstallation/chapter12.1.tex}

\input{AssemblyAndInstallation/chapter12.2.tex}

\input{AssemblyAndInstallation/chapter12.3.tex}

\input{AssemblyAndInstallation/chapter12.4.tex}

\input{AssemblyAndInstallation/chapter12.5.tex}



==> maintex/authors.tex <==
\newcommand{\ANL}{1}
\newcommand{\APC}{2}
\newcommand{\BNU}{3}
\newcommand{\CIAE}{4}
\newcommand{\CPPM}{5}
\newcommand{\CQU}{6}
\newcommand{\CUPrague}{7}
\newcommand{\DGUT}{8}
\newcommand{\ECUST}{9}
\newcommand{\EKUT}{10}
\newcommand{\FZJ}{11}
\newcommand{\GXU}{12}
\newcommand{\Hamburg}{13}
\newcommand{\HIT}{14}
\newcommand{\IHEGCAGS}{15}
\newcommand{\IHEP}{16}
\newcommand{\INFNFerrara}{17}
\newcommand{\INFNLNF}{18}
\newcommand{\INFNMI}{19}
\newcommand{\INFNMiB}{20}
\newcommand{\INFNMiBP}{21}
\newcommand{\INFNMiBU}{22}
\newcommand{\INFNPD}{23}
\newcommand{\INFNPG}{24}
\newcommand{\INFNRoma}{25}
\newcommand{\INRRAS}{26}
\newcommand{\IPHC}{27}
\newcommand{\JGUMainz}{28}
\newcommand{\JINR}{29}
\newcommand{\JLU}{30}
\newcommand{\LLRParis}{31}
\newcommand{\Nankai}{32}
\newcommand{\NCEPU}{33}
\newcommand{\NCTU}{34}
\newcommand{\NJU}{35}
\newcommand{\NTU}{36}
\newcommand{\NUU}{37}
\newcommand{\PKU}{38}
\newcommand{\PUCC}{39}
\newcommand{\RWTHAC}{40}
\newcommand{\SDU}{41}
\newcommand{\SichuanU}{42}
\newcommand{\SJTU}{43}
\newcommand{\SUBATECH}{44}
\newcommand{\SYSU}{45}
\newcommand{\Tsinghua}{46}
\newcommand{\TUM}{47}
\newcommand{\UCAS}{48}
\newcommand{\ULB}{49}
\newcommand{\UMDG}{50}
\newcommand{\UMDP}{51}
\newcommand{\UNIPD}{52}
\newcommand{\UOULU}{53}
\newcommand{\USTC}{54}
\newcommand{\WHU}{55}
\newcommand{\WuYi}{56}
\newcommand{\XJTU}{57}
\newcommand{\XMU}{58}
\newcommand{\YerPhI}{59}
\author[\ANL]{Zelimir Djurcic}
\author[\ANL]{Vic Guarino}
\author[\APC]{Anatael Cabrera}
\author[\APC]{Hervé de Kerret}
\author[\APC]{Cristina Volpe}
\author[\BNU]{Xinheng Guo}
\author[\BNU]{Jing Xu}
\author[\CIAE]{Shouyang Hu}
\author[\CIAE]{Hanxiong Huang}
\author[\CIAE]{Siyu Jian}
\author[\CIAE]{Xiaomei Li}
\author[\CIAE]{Xinglong Li}
\author[\CIAE]{Hao Liang}
\author[\CIAE]{Jie Ren}
\author[\CIAE]{Xichao Ruan}
\author[\CIAE]{Minshan Zheng}
\author[\CIAE]{Jing Zhou}
\author[\CPPM]{Jose Busto}
\author[\CPPM]{Damien Dornic}
\author[\CQU]{Jiaxing Li}
\author[\CQU]{Dongmei Xia}
\author[\CQU]{Wenxiong Zhou}
\author[\CUPrague]{Rupert Leitner}
\author[\CUPrague]{Viktor Pec}
\author[\CUPrague]{Bedrich Roskovec}
\author[\CUPrague]{Vit Vorobel}
\author[\DGUT]{Pingping Chen}
\author[\DGUT]{Li Kang}
\author[\DGUT]{Ruiting Lei}
\author[\DGUT]{Shanfeng Li}
\author[\DGUT]{Yi Li}
\author[\DGUT]{Shengxin Lin}
\author[\DGUT]{Bin Ren}
\author[\DGUT]{Caishen Wang}
\author[\DGUT]{Yadong Wei}
\author[\DGUT]{Lei Yang}
\author[\DGUT]{Chiye Yu}
\author[\DGUT]{Zhijian Zhang}
\author[\DGUT]{Hua Zheng}
\author[\ECUST]{Fengpeng An}
\author[\EKUT]{Tobias Lachenmaier}
\author[\EKUT]{Alexander Tietzsch}
\author[\FZJ]{Christian Grewing}
\author[\FZJ]{Michael Karagounis}
\author[\FZJ]{Andre Kruth}
\author[\FZJ]{Pavithra Muralidharan}
\author[\FZJ]{Nina Parkalian}
\author[\FZJ]{Markus Robens}
\author[\FZJ]{Stefan van Waasen}
\author[\FZJ]{Yu Yao}
\author[\FZJ]{Ugur Yegin}
\author[\GXU]{Can Fang}
\author[\GXU]{Daojin Hong}
\author[\GXU]{Jingjing Liang}
\author[\GXU]{Hongbang Liu}
\author[\GXU]{Xiangdong Ruan}
\author[\Hamburg]{Daniel Bick}
\author[\Hamburg]{Caren Hagner}
\author[\Hamburg]{Markus Kaiser}
\author[\Hamburg]{Sebastian Lorenz}
\author[\Hamburg]{Björn Wonsak}
\author[\HIT]{Lei Huo}
\author[\HIT]{Jianli Liu}
\author[\HIT]{Guoli Wang}
\author[\HIT]{Jingbo Zhang}
\author[\IHEGCAGS]{Haonan Gan}
\author[\IHEGCAGS]{Chuan Lu}
\author[\IHEGCAGS]{Yufei Xi}
\author[\IHEP]{Guangpeng An}
\author[\IHEP]{Xiao Cai}
\author[\IHEP]{Guofu Cao}
\author[\IHEP]{Jun Cao}
\author[\IHEP]{Jinfan Chang}
\author[\IHEP]{Mingming Chen}
\author[\IHEP]{Xuan Chen}
\author[\IHEP]{Yaping Cheng}
\author[\IHEP]{Ziyan Deng}
\author[\IHEP]{Yayun Ding}
\author[\IHEP]{Jian Fang}
\author[\IHEP]{Marco Grassi}
\author[\IHEP]{Minghao Gu}
\author[\IHEP]{Mengyun Guan}
\author[\IHEP]{Wanlei Guo}
\author[\IHEP]{Ziguo Han}
\author[\IHEP]{Jiajun Hao}
\author[\IHEP]{Miao He}
\author[\IHEP]{Yuekun Heng}
\author[\IHEP]{Shaojing Hou}
\author[\IHEP]{Jun Hu}
\author[\IHEP]{Tao Hu}
\author[\IHEP]{Wei Hu}
\author[\IHEP]{Soeren Jetter}
\author[\IHEP]{Xiaolu Ji}
\author[\IHEP]{Xiaoshan Jiang}
\author[\IHEP]{Bowen Kan}
\author[\IHEP]{Xiangcui Lei}
\author[\IHEP]{Fei Li}
\author[\IHEP]{Nan Li}
\author[\IHEP]{Weidong Li}
\author[\IHEP]{Weiguo Li}
\author[\IHEP]{Xiaonan Li}
\author[\IHEP]{Yufeng Li}
\author[\IHEP]{Tao Lin}
\author[\IHEP]{Gang Liu}
\author[\IHEP]{Jinchang Liu}
\author[\IHEP]{Shulin Liu}
\author[\IHEP]{Haoqi Lu}
\author[\IHEP]{Jiashu Lu}
\author[\IHEP]{Junguang Lu}
\author[\IHEP]{Fengjiao Luo}
\author[\IHEP]{Qiumei Ma}
\author[\IHEP]{Si Ma}
\author[\IHEP]{Xiaoyan Ma}
\author[\IHEP]{Jian Min}
\author[\IHEP]{Zhe Ning}
\author[\IHEP]{Fazhi Qi}
\author[\IHEP]{Sen Qian}
\author[\IHEP]{Xiaohui Qian}
\author[\IHEP]{Zhonghua Qin}
\author[\IHEP]{Jingyan Shi}
\author[\IHEP]{Gongxing Sun}
\author[\IHEP]{Xilei Sun}
\author[\IHEP]{Yongzhao Sun}
\author[\IHEP]{Ruiguang Wang}
\author[\IHEP]{Yifang Wang}
\author[\IHEP]{Zheng Wang}
\author[\IHEP]{Zhigang Wang}
\author[\IHEP]{Zhimin Wang}
\author[\IHEP]{Wei Wei}
\author[\IHEP]{Liangjian Wen}
\author[\IHEP]{Yijie Wen}
\author[\IHEP]{Zhi Wu}
\author[\IHEP]{Jingkai Xia}
\author[\IHEP]{Yuguang Xie}
\author[\IHEP]{Jilei Xu}
\author[\IHEP]{Lingyu Xu}
\author[\IHEP]{Baojun Yan}
\author[\IHEP]{Xiongbo Yan}
\author[\IHEP]{Changgen Yang}
\author[\IHEP]{Mei Ye}
\author[\IHEP]{Boxiang Yu}
\author[\IHEP]{Zeyuan Yu}
\author[\IHEP]{Shan Zeng}
\author[\IHEP]{Tingxuan Zeng}
\author[\IHEP]{Liang Zhan}
\author[\IHEP]{Chengcai Zhang}
\author[\IHEP]{Guoqing Zhang}
\author[\IHEP]{Jiawen Zhang}
\author[\IHEP]{Jie Zhang}
\author[\IHEP]{Kun Zhang}
\author[\IHEP]{Peng Zhang}
\author[\IHEP]{Xiaomei Zhang}
\author[\IHEP]{Xuan Zhang}
\author[\IHEP]{Yinhong Zhang}
\author[\IHEP]{Yongjie Zhang}
\author[\IHEP]{Yongpeng Zhang}
\author[\IHEP]{Jie Zhao}
\author[\IHEP]{Mei Zhao}
\author[\IHEP]{Tianchi Zhao}
\author[\IHEP]{Yubin Zhao}
\author[\IHEP]{Weili Zhong}
\author[\IHEP]{Li Zhou}
\author[\IHEP]{Shun Zhou}
\author[\IHEP]{Kejun Zhu}
\author[\IHEP]{Honglin Zhuang}
\author[\IHEP]{Jiaheng Zou}
\author[\INFNFerrara]{Marica Baldoncini}
\author[\INFNFerrara]{Giovanni Fiorentini}
\author[\INFNFerrara]{Fabio Mantovani}
\author[\INFNFerrara]{Michele Montuschi}
\author[\INFNFerrara]{Barbara Ricci}
\author[\INFNFerrara]{Virginia Strati}
\author[\INFNLNF]{Alessandro Paoloni}
\author[\INFNLNF]{Lucia Votano}
\author[\INFNMI]{Vito Antonelli}
\author[\INFNMI]{Augusto Brigatti}
\author[\INFNMI]{Davide D'Angelo}
\author[\INFNMI]{Richard Ford}
\author[\INFNMI]{Marco Giammarchi}
\author[\INFNMI]{Paolo Lombardi}
\author[\INFNMI]{Livia Ludhova}
\author[\INFNMI]{Emanuela Meroni}
\author[\INFNMI]{Lino Miramonti}
\author[\INFNMI]{Sergio Parmeggiano}
\author[\INFNMI]{Gioacchino Ranucci}
\author[\INFNMI]{Alessandra Re}
\author[\INFNMI]{Paolo Saggese}
\author[\INFNMiB]{Roberto Gaigher}
\author[\INFNMiBP]{Sara Boarin}
\author[\INFNMiBP]{Antonio Cammi}
\author[\INFNMiBP]{Matteo Zanetti}
\author[\INFNMiBU]{Giovanni Baccolo}
\author[\INFNMiBU]{Davide Chiesa}
\author[\INFNMiBU]{Massimiliano Clemenza}
\author[\INFNMiBU]{Massimiliano Nastasi}
\author[\INFNMiBU]{Stefano Pozzi}
\author[\INFNMiBU]{Ezio Previtali}
\author[\INFNMiBU]{Monica Sisti}
\author[\INFNPD]{Marco Bellato}
\author[\INFNPD]{Stefano Dusini}
\author[\INFNPD]{Ivano Lippi}
\author[\INFNPD]{Guang Meng}
\author[\INFNPD]{Mauro Mezzetto}
\author[\INFNPD]{Luca Stanco}
\author[\INFNPG]{Fausto Ortica}
\author[\INFNPG]{Nicomede Pelliccia}
\author[\INFNPG]{Aldo Romani}
\author[\INFNRoma]{Stefano Mari}
\author[\INFNRoma]{Giuseppe Salamanna}
\author[\INRRAS]{Leonid Bezrukov}
\author[\INRRAS]{Evgeny Doroshkevich}
\author[\INRRAS]{Svetlana Krokhaleva}
\author[\INRRAS]{Bayarto Lubsandorzhiev}
\author[\INRRAS]{Sultim Lubsandorzhiev}
\author[\INRRAS]{Vladimir Lyashuk}
\author[\INRRAS]{Valery Sinev}
\author[\INRRAS]{Igor Tkachev}
\author[\INRRAS]{Evgeny Yanovich}
\author[\IPHC]{Thomas Adam}
\author[\IPHC]{Eric Baussan}
\author[\IPHC]{Timothée Brugière}
\author[\IPHC]{Marcos Dracos}
\author[\IPHC]{Gérard Gaudiot}
\author[\IPHC]{Cécile Jollet}
\author[\IPHC]{Anselmo Meregaglia}
\author[\IPHC]{Pascal Poussot}
\author[\IPHC]{Jacky Schuler}
\author[\IPHC]{Jacques Wurtz}
\author[\JGUMainz]{Paul Hackspacher}
\author[\JGUMainz]{Michael Wurm}
\author[\JINR]{Nikolay Anfimov}
\author[\JINR]{Artem Chukanov}
\author[\JINR]{Sergey Dmitrievsky}
\author[\JINR]{Maria Dolgareva}
\author[\JINR]{Dmitry Fedoseev}
\author[\JINR]{Andrey Formozov}
\author[\JINR]{Maxim Gonchar}
\author[\JINR]{Yuri Gornushkin}
\author[\JINR]{Vasily Gromov}
\author[\JINR]{Denis Korablev}
\author[\JINR]{Alexey Krasnoperov}
\author[\JINR]{Zinovy Krumshteyn}
\author[\JINR]{Nikolay Morozov}
\author[\JINR]{Dmitry Naumov}
\author[\JINR]{Elena Naumova}
\author[\JINR]{Igor Nemchenok}
\author[\JINR]{Alexander Olshevskiy}
\author[\JINR]{Taras Rezinko}
\author[\JINR]{Arseniy Rybnikov}
\author[\JINR]{Andrey Sadovsky}
\author[\JINR]{Alexandr Selyunin}
\author[\JINR]{Oleg Smirnov}
\author[\JINR]{Dmitriy Taichenachev}
\author[\JLU]{Jingbin Lu}
\author[\LLRParis]{Margherita Buizza Avanzini}
\author[\LLRParis]{Olivier Drapier}
\author[\LLRParis]{Michel Gonin}
\author[\LLRParis]{Matthieu Licciardi}
\author[\LLRParis]{Thomas Mueller}
\author[\Nankai]{Xinying Li}
\author[\Nankai]{Jinyan Liu}
\author[\Nankai]{Yuanyuan Liu}
\author[\Nankai]{Cui Wang}
\author[\Nankai]{Yin Xu}
\author[\Nankai]{Yujiao Yang}
\author[\Nankai]{Chunxu Yu}
\author[\Nankai]{Xiangyu Zheng}
\author[\NCEPU]{Yixue Chen}
\author[\NCEPU]{Ran Han}
\author[\NCEPU]{Fan Lu}
\author[\NCEPU]{Xubo Ma}
\author[\NCTU]{Kuo-Lun Jen}
\author[\NCTU]{Guey-Lin Lin}
\author[\NCTU]{Yen-Hsun Lin}
\author[\NCTU]{Chia-Hao Wu}
\author[\NJU]{Dewen Cao}
\author[\NJU]{Shenjian Chen}
\author[\NJU]{Xiaozhong Huang}
\author[\NJU]{Ming Qi}
\author[\NJU]{Hongxin Wang}
\author[\NJU]{Wenwen Wang}
\author[\NJU]{Haibo Yang}
\author[\NJU]{Yuzhen Yang}
\author[\NJU]{Guangyou Yu}
\author[\NTU]{Simon Blyth}
\author[\NTU]{Yee Hsiung}
\author[\NTU]{Bei-Zhen Hu}
\author[\NTU]{Hsiao-Ru Pan}
\author[\NTU]{Yu-Chen Tung}
\author[\NUU]{Yun Chang}
\author[\NUU]{Chung-Hsiang Wang}
\author[\PKU]{Yajun Mao}
\author[\PKU]{Hao Qiao}
\author[\PKU]{Siguang Wang}
\author[\PKU]{Ying Yuan}
\author[\PUCC]{Marco Aurelio Díaz}
\author[\PUCC]{Yury Malyshkin}
\author[\PUCC]{Juan Pedro Ochoa-Ricoux}
\author[\RWTHAC]{Christoph Genster}
\author[\RWTHAC]{Florian Lenz}
\author[\RWTHAC]{Michael Soiron}
\author[\RWTHAC]{Achim Stahl}
\author[\RWTHAC]{Jochen Steinmann}
\author[\RWTHAC]{Marcel Weifels}
\author[\RWTHAC]{Christopher Wiebusch}
\author[\SDU]{Quanyou Chen}
\author[\SDU]{Xingtao Huang}
\author[\SDU]{Chao Li}
\author[\SDU]{Teng Li}
\author[\SDU]{Meng Wang}
\author[\SDU]{Qun Wu}
\author[\SDU]{Mengting Yang}
\author[\SichuanU]{Xiao Fang}
\author[\SichuanU]{Chaowen Yang}
\author[\SichuanU]{Rong Zhou}
\author[\SJTU]{Franco Giuliani}
\author[\SJTU]{Jianglai Liu}
\author[\SJTU]{Feiyang Zhang}
\author[\SJTU]{Tao Zhang}
\author[\SJTU]{Yuanyuan Zhang}
\author[\SUBATECH]{Frédéric Yermia}
\author[\SYSU]{Zhibing Li}
\author[\SYSU]{Hu Liu}
\author[\SYSU]{Jian Tang}
\author[\SYSU]{Wei Wang}
\author[\SYSU]{Steven Chan-Fai Wong}
\author[\SYSU]{Zhengyun You}
\author[\SYSU]{Honghao Zhang}
\author[\SYSU]{Yumei Zhang}
\author[\Tsinghua]{Shaomin Chen}
\author[\Tsinghua]{Zhi Deng}
\author[\Tsinghua]{Guanghua Gong}
\author[\Tsinghua]{Hui Gong}
\author[\Tsinghua]{Liping Lei}
\author[\Tsinghua]{Fule Li}
\author[\Tsinghua]{Gang Shi}
\author[\Tsinghua]{Yongjiu Shi}
\author[\Tsinghua]{Yi Wang}
\author[\Tsinghua]{Yuanqing Wang}
\author[\Tsinghua]{Zhe Wang}
\author[\Tsinghua]{Zongyi Wang}
\author[\Tsinghua]{Zhenxiong Yuan}
\author[\Tsinghua]{Pan Zeng}
\author[\Tsinghua]{Yan Zhou}
\author[\Tsinghua]{Liang Zong}
\author[\TUM]{Marianne Göger-Neff}
\author[\TUM]{Dominikus Hellgartner}
\author[\TUM]{Lothar Oberauer}
\author[\TUM]{Sabrina Prummer}
\author[\TUM]{Julia Sawatzki}
\author[\UCAS]{Shi Chen}
\author[\UCAS]{Qian Liu}
\author[\UCAS]{Yuning Zhang}
\author[\UCAS]{Yangheng Zheng}
\author[\ULB]{Barbara Clerbaux}
\author[\ULB]{Laurent Favart}
\author[\ULB]{Yifan Yang}
\author[\UMDG]{William McDonough}
\author[\UMDG]{Scott Wipperfurth}
\author[\UMDP]{Xiangdong Ji}
\author[\UMDP]{Mengjiao Xiao}
\author[\INFNPD,\UNIPD]{Riccardo Brugnera}
\author[\INFNPD,\UNIPD]{Alberto Garfagnini}
\author[\INFNPD,\UNIPD]{Chiara Sirignano}
\author[\UOULU]{Timo Enqvist}
\author[\UOULU]{Pasi Kuusiniemi}
\author[\USTC]{Qi An}
\author[\USTC]{Wenju Huo}
\author[\USTC]{Di Jiang}
\author[\USTC]{Hao Liang}
\author[\USTC]{Qin Liu}
\author[\USTC]{Shubin Liu}
\author[\USTC]{Haiping Peng}
\author[\USTC]{Yongjie Sun}
\author[\USTC]{Nan Zhou}
\author[\WHU]{Hao Cai}
\author[\WHU]{Xuefeng Ding}
\author[\WHU]{Xingchen Ye}
\author[\WHU]{Zhenyu Zhang}
\author[\WHU]{Xiang Zhou}
\author[\WHU]{Haiwen Zhu}
\author[\WuYi]{Donghua Fan}
\author[\WuYi]{Yongbing Long}
\author[\WuYi]{Yi Wang}
\author[\WuYi]{Guorong Zhou}
\author[\XJTU]{Yuhang Guo}
\author[\XJTU]{Zhipeng Lv}
\author[\XJTU]{Qingmin Zhang}
\author[\XMU]{Shu Luo}
\author[\YerPhI]{Ara Ioannisian}
\author[\YerPhI]{Daniel Ioannisyan}
\author[\YerPhI]{Narine Kazarian}
\author[\YerPhI]{Davit Mayilyan}
\affil[\ANL]{Argonne National Laboratory, Argonne, IL, USA}
\affil[\APC]{Astro-Particle Physics Laboratory (CNRS/CEA/Paris7/Observatoire de Paris), Paris, France}
\affil[\BNU]{Beijing Normal University, Beijing, China}
\affil[\CIAE]{China Institute of Atomic Energy, Beijing, China}
\affil[\CPPM]{Centre de Physique des Particules de Marseille, Marseille, France}
\affil[\CQU]{Chongqing University, Chongqing, China}
\affil[\CUPrague]{Charles University, Faculty of Mathematics and Physics, Prague, Czech Republic}
\affil[\DGUT]{Dongguan University of Technology, Dongguan, China}
\affil[\ECUST]{East China University of Science and Technology, Shanghai, China}
\affil[\EKUT]{Eberhard Karls Universität Tübingen, Physikalisches Institut, Tübingen, Germany}
\affil[\FZJ]{Forschungszentrum Jülich GmbH, Central Institute of Engineering, Electronics and Analytics - Electronic Systems(ZEA-2), Jülich, Germany}
\affil[\GXU]{Guangxi University, Nanning, China}
\affil[\Hamburg]{Institute of Experimental Physics, University of Hamburg, Hamburg, Germany}
\affil[\HIT]{Harbin Institute of Technology, Harbin, China}
\affil[\IHEGCAGS]{Institute of Hydrogeology and Environmental Geology, Chinese Academy of Geological Sciences, Shijiazhuang, China}
\affil[\IHEP]{Institute of High Energy Physics, Beijing, China}
\affil[\INFNFerrara]{Department of Physics and Earth Science, University of Ferrara and INFN Sezione di Ferrara, Ferrara, Italy}
\affil[\INFNLNF]{Laboratori Nazionali di Frascati dell'INFN, Roma, Italy}
\affil[\INFNMI]{INFN Sezione di Milano and Dipartimento di Fisica dell Università di Milano, Milano, Italy}
\affil[\INFNMiB]{INFN Milano Bicocca, Milano, Italy}
\affil[\INFNMiBP]{INFN Milano Bicocca and Politecnico di Milano, Department of Energy CeSNEF (Enrico Fermi Center for Nuclear Studies), Milano, Italy}
\affil[\INFNMiBU]{INFN Milano Bicocca and Department of Physics “G. Occhialini”, University of Milano Bicocca, Milano, Italy}
\affil[\INFNPD]{INFN Sezione di Padova, Padova, Italy}
\affil[\INFNPG]{INFN and University of Perugia - Department of Chemistry, Biology and Biotechnology, Perugia, Italy}
\affil[\INFNRoma]{University of Roma Tre and INFN Sezione Roma Tre, Roma, Italy}
\affil[\INRRAS]{Institute for Nuclear Research of the Russian Academy of Sciences, Moscow, Russia}
\affil[\IPHC]{Institut Pluridisciplinaire Hubert Curien, Université de Strasbourg, CNRS/IN2P3, Strasbourg, France}
\affil[\JGUMainz]{Institute of Physics and EC PRISMA, Johannes-Gutenberg University Mainz, Mainz, Germany}
\affil[\JINR]{Joint Institute for Nuclear Research, Dubna, Russia}
\affil[\JLU]{Jilin University, Changchun, China}
\affil[\LLRParis]{Leprince-Ringuet Laboratory Ecole Polytechnique, Palaiseau Cedex, France}
\affil[\Nankai]{Nankai University, Tianjin, China}
\affil[\NCEPU]{North China Electric Power University, Beijing, China}
\affil[\NCTU]{Institute of Physics National Chiao-Tung University, Hsinchu, Taiwan, China}
\affil[\NJU]{Nanjing University, Nanjing, China}
\affil[\NTU]{Department of Physics, National Taiwan University, Taipei, Taiwan, China}
\affil[\NUU]{National United University, Miao-Li, Taiwan, China}
\affil[\PKU]{School of Physics, Peking University, Beijing, China}
\affil[\PUCC]{Instituto de Fisica, Pontificia Universidad Católica de Chile, Santiago, Chile}
\affil[\RWTHAC]{III. Physikalisches Institut B, RWTH Aachen University, Aachen, Germany}
\affil[\SDU]{Shandong University, Jinan, China}
\affil[\SichuanU]{Sichuan University, Chengdu, China}
\affil[\SJTU]{Shanghai Jiao Tong University, Shanghai, China}
\affil[\SUBATECH]{SUBATECH, CNRS/IN2P3, Université de Nantes, Ecole des Mines de Nantes, Nantes, France}
\affil[\SYSU]{Sun Yat-Sen University, Guangzhou, China}
\affil[\Tsinghua]{Tsinghua University, Beijing, China}
\affil[\TUM]{Technical University of Munich, Garching, Germany}
\affil[\UCAS]{University of Chinese Academy of Sciences, Beijing, China}
\affil[\ULB]{Université Libre de Bruxelles, Brussels, Belgium}
\affil[\UMDG]{Department of Geology, University of Maryland, College Park, MD 20742, USA}
\affil[\UMDP]{Department of Physics, University of Maryland, College Park, MD, USA}
\affil[\UNIPD]{Dipartimento di Fisica e Astronomia dell'Università di Padova, Padova, Italy}
\affil[\UOULU]{Oulu Southern Institute, University of Oulu, Pyhasalmi, Finland}
\affil[\USTC]{University of Science and Technology of China, Hefei, China}
\affil[\WHU]{Wuhan University, Wuhan, China}
\affil[\WuYi]{Wuyi University, Jiangmen, China}
\affil[\XJTU]{Xi'an Jiaotong University, Xi'an, China}
\affil[\XMU]{Xiamen University, Xiamen, China}
\affil[\YerPhI]{Yerevan Physics Institute, Yerevan, Armenia}


==> maintex/frontmatter.tex <==
% title page
\cleardoublepage
\title{JUNO Conceptual Design Report}
\date{\today}
\pagestyle{empty}
\makeatletter
\begin{titlepage}
\begin{center}
\vspace{3cm}

{\normalfont\sffamily\Huge\bfseries\scshape \@title}
\vspace{1cm}

{\Large \@date}
\vspace{2cm}

\includegraphics[width=0.65\textwidth]{figures/junologo.jpg}
\vspace{1cm}

\end{center}
\end{titlepage}
\makeatother


% Abstract
\cleardoublepage
\pagestyle{empty}
\makeatletter
\input{maintex/abstract}   
\makeatother

% Detail Author List
\cleardoublepage
\pagestyle{empty}
\input{maintex/authors}   
\makeatletter
\begin{titlepage}
\begin{center}

{\normalfont\sffamily\Huge\bfseries\scshape JUNO Collaboration}
\vspace{1cm}

{\footnotesize \@author}

\end{center}
\end{titlepage}
\makeatother


% Table of contents
\cleardoublepage
\setcounter{page}{1}
\pagestyle{plain}
\renewcommand{\thepage}{\roman{page}}
\setcounter{tocdepth}{3}
\addtocontents{toc}{\protect{\pdfbookmark[0]{Table of Contents}{toc}}}
\textsf{\tableofcontents}


% Acronym list, needs nomencl
%\cleardoublepage
%\printnomenclature

% Table of Figures
\cleardoublepage
\phantomsection
\addcontentsline{toc}{chapter}{\listfigurename}
\textsf{\listoffigures}

% Table of Tables
\cleardoublepage
\phantomsection
\addcontentsline{toc}{chapter}{\listtablename}
%\pdfbookmark[0]{List of Tables}{lot}
\textsf{\listoftables}


